The Synergy of Speculative Decoding and Batching in Serving Large Language Models

Large Language Models (LLMs) like GPT are state-of-the-art text generation models that provide significant assistance in daily routines. However, LLM execution is inherently sequential, since they only produce one token at a time, thus incurring low hardware utilization on modern GPUs. Batching and speculative decoding are two techniques to improve GPU hardware utilization in LLM inference. To study their synergy, we implement a prototype implementation and perform an extensive characterization analysis on various LLM models and GPU architectures. We observe that the optimal speculation length depends on the batch size used. We analyze the key observation and build a quantitative model to explain it. Based on our analysis, we propose a new adaptive speculative decoding strategy that chooses the optimal speculation length for different batch sizes. Our evaluations show that our proposed method can achieve equal or better performance than the state-of-the-art speculation decoding schemes with fixed speculation length.

==> contents/analysis.tex <==
\section{Analysis}

In this section, we will analyze the reason behind our observation. The notations are listed in Table~\ref{tab:notation}. 
Th e total runtime of speculative decoding consists of two parts, namely the runtime of LLM and SSM, which can be formulated as

\begin{equation}
t = \frac{N \cdot t_L(B, s)}{l(s) + 1} + \frac{N \cdot s \cdot t_S(B, 2)}{l(s) + 1}
\end{equation}


\begin{table}[h]
    \centering
    \small
    \caption{Notations}
    \begin{tabular}{ p{0.2\linewidth} | p{0.7\linewidth} }
        \toprule
       $N$ & Total number of tokens to be generated \\ \midrule
       $s$ & Number of speculated tokens in each speculative step \\ \midrule
       $t_{\{L, S\}}(B, s)$ & Runtime of the large/small model with batchsize=$B$ and query length $s$ \\ \midrule
       $l(s)$ & Expected number of correct tokens generated in each speculative step \\ \midrule
       $E_i$ & Indicator random variable, equal to $1$ when the $i$-th token is correct, $0$ otherwise \\
       \bottomrule
    \end{tabular}
    \label{tab:notation}
\end{table}

\paragraph{Runtime of the LLM} LLM is used to verify the tokens generated by the SSM. The number of calls to the LLM $\frac{N}{l(s) + 1}$ is determined by the total number of tokens to be generated $N$ and the average number of correct tokens generated by SSM $l(s)$. Because the LLM will always generate an extra new token, either by correcting a wrong prediction, or looking ahead if all tokens are speculated correctly, the effective number of tokens generated in each step is ${l(s) + 1}$.


Intuitively, $l(s)$ is non-decreasing and sub-linear. It is because we can decompose $l(s)$ as following:

\begin{equation}
    l(s)=\sum_{i=1}^{s} p(\bigwedge_{j=1}^i E_i)
\end{equation}

Each term in the summation is non-negative. As $s$ increases, it is harder to make correct speculation, so the probability $p$ will decrease rapidly.

Empirically, $l(s)$ can be approximated by a polynomial function $l(s)= c\cdot s^\gamma$, where $s<1$, as shown in Figure~\ref{fig:seqlen-time}.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/expected-len.pdf}
    \caption{How $l(s)$ scales with $s$, which can be approximated by a sublinear power function $c\cdot s^\gamma$, where $\gamma < 1$.}
    \label{fig:expected-len}
\end{figure}

Meanwhile, $t_L(B, s)$ depends on the hardware and model implementations.
We measured the runtime of OPT-6.7B on an RTX 3090 GPU, and the result is shown in Figure~\ref{fig:seqlen-time}. The runtime curves are approximately step functions. The first jump of the curve of $B=1$ is when $s=64$, while that of $B=8$ jumps up much earlier when $s=8$. For simplicity, we approximate $t_L(B, s)$ as linear functions with different slopes $t_L(B, s) = c_B s + b$. 

\begin{figure}
    \centering
    \includegraphics[width=0.2\linewidth]{figures/seqlen-time.pdf}
    \caption{How $t_L(B, s)$ scales with $s$ for different $B$-s, which can be approximated by a linear function.}
    \label{fig:seqlen-time}
\end{figure}

\paragraph{Runtime of the SSM}
In practice, we usually also need to consider the second term, i.e. the runtime of the small model. For a fixed $B$, $t_S(B,1)$ is a constant, and the constant is also increasing with $B$. Therefore we can merge it with the linear term in the runtime of LLM.


\paragraph{Optimal speculation length} Based on the analysis above, the total runtime can be written as

\begin{equation}
t = \frac{N \cdot t_L(B, s)}{l(s) + 1} + \frac{N \cdot s \cdot t_S(B, 1)}{l(s) + 1} \approx N \frac{c_B \cdot s + b}{c\cdot s^\gamma + 1} 
\end{equation}

The minimum point of this function $s^*$ is where the derivative of $t$ is zero, i.e. $\frac{\partial t}{\partial s} = 0$. And we have

\begin{equation}
\frac{\partial t}{\partial s} = N\frac{c_B(c\cdot s^\gamma + 1) - (c_B \cdot s + b)\cdot c \gamma s^{\gamma - 1}}{(c\cdot s^\gamma + 1)^2}
\end{equation}

It is zero when the numerator is zero, which can be written as $(1-\gamma)c_B \cdot c s^\gamma - c\cdot b \cdot \gamma s^{\gamma - 1} + c_B$, which is monotonically increasing with respect to both $s$ and $B$. Therefore, with larger $c_B$, $s^*$ needs to be smaller in order to have the derivative as zero. 
